Semi-Streaming Algorithms for Submodular Maximization under Random Arrival Order

We study random order semi-streaming algorithms for submodular maximization under a wide range of combinatorial constraint classes, including matroids, matroid $p$-parity, $p$-exchange systems and $p$-systems. For most of these classes of constraints, our results are the first improvement over what is known to be achievable for adversarial order. For matroids, matching and $p$-matchoids, previous random order results were known, and we improve over some of these as well. In the case of matroids, our improved results show a separation between adversarial and random order semi-streaming algorithms, and exponentially improve the number of passes necessary for getting $1 - 1/e - \varepsilon$ approximation for maximizing a monotone submodular function subject to a matroid constraint. We also prove a new hardness result showing a similar separation for $p$-systems. Our results are based on two new technical tools. One tool provides a general way to translate offline algorithms for many classes of constraints into random order semi-streaming algorithms. The other tool is a semi-streaming variant of a recently proposed offline algorithm for matroid constraints.

==> conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}

\mf{Do we need a conclusion at all? I think this is not necessary, unless someone has an open problem they really want to pose, or something like that.}

==> main-alg.tex <==
\section{Single Pass Semi-streaming Algorithm with Boosting}\label{sec:mainAlg}

\siyue{TODO: Make the proof of Section 5.2 work for the general Alg \ref{alg:iid} and add the short list proof after it.}

\subsection{Continuous analysis for i.i.d. arrival}
To gain some intuition of the algorithm, we start with a slightly different setting. Let $\ell$ be a positive integer. Suppose at each time step from $1$ to $\ell$, an element $v\in E$ arrives uniformly at random with probability at least $\frac{1}{\ell}$ and the elements arrive independently across all time steps. We show that \Cref{alg:iid} achieves the desired inequality as in \Cref{prop:main}. 
% \begin{algorithm}
% \caption{\textsc{Single-Pass with i.i.d. Arrival}} \label{alg:iid}
% \KwIn{A basis $A$ and a value $h\in [0,1/e]$}
% \For{$t = 1$ \KwTo $\ell$}
% {   A uniformly random element $v\in OPT$ arrives with probability at least $\frac{1}{\ell}$.\\
%     Let $h(t)=h\cdot e^{t/\ell}$.\\
%     Pick $u\in A$ such that $A-u+v\in\cal{I}$ and $F(h(t)\cdot \characteristic_{A-u+v})$ is maximized.\\
%     \If{$F(h(t)\cdot \characteristic_{A-u+v})>F(h(t)\cdot \characteristic_{A})$}
%     {
%     Let $A\gets A-u+v$.
%     }
% }
% \Return $A$.
% \end{algorithm}

\begin{algorithm}
\caption{\textsc{Offline Random Local Search}} \label{alg:iid}
\KwIn{An initial basis $A$ and a value $h\in [0,1/e]$}
\For{$t = 1$ \KwTo $\ell$}
{   Sample a random set $R\subseteq \mathcal{N}$ where every element appears independently uniformly at random with probability at least $1/\ell$.\\
    Let $h(t)=h\cdot e^{t/\ell}$.\\
    Pick $v\in R$ and $u\in A$ such that $A-u+v\in\cal{I}$ and $F(h(t)\cdot \characteristic_{A-u+v})$ is maximized.\\
    \If{$F(h(t)\cdot \characteristic_{A-u+v})>F(h(t)\cdot \characteristic_{A})$}
    {
    Let $A\gets A-u+v$.
    }
}
\Return $A$.
\end{algorithm}



\siyue{Is there a better way to write this Proposition? Maybe not use $\gtrsim$...}
\begin{proposition}
    For sufficiently large $\ell$, \Cref{alg:iid} takes an input $A\in \mathcal{I}$ and outputs $S\in \mathcal{I}$ such that
\[
\ex{[F(e\cdot h\cdot \characteristic_{S})]}-F(h\cdot \characteristic_{A})\cdot e^{-h \cdot (e-1)}\gtrsim (1-e^{-h \cdot (e-1)})\cdot F(OPT).
\]
\end{proposition}
\begin{proof}
For easier analysis, we think of the time steps as continuous. Denote the sets $A, R$ at time $t$ as $A(t), R(t)$, respectively. Denote as $v(t)\in R(t)$ and $u(t)\in A(t)$ the pair of random elements we swap at time $t$ (let $u(t)=v(t)$ if we do not carry out the swap). For analysis of the gain of $F$ in one unit time step of the algorithm, we assume $A(t)$ is deterministic and the randomness comes from $R(t)$. By the chain rule,
    \begin{equation}\label{eq:chain_rule}
            \begin{aligned}
        \frac{d\, F(h(t)\cdot \characteristic_{A(t)})}{d\, t}
        =& \Big\langle \nabla F(h(t)\cdot\characteristic_{A(t)}),\ \characteristic_{A(t)}\Big\rangle\cdot \frac{d\, h(t)}{d\, t}+ \Big\langle\nabla F(h(t)\cdot\characteristic_{A(t)}),\ \frac{d\, \characteristic_{A(t)}}{d\, t}\Big\rangle \cdot h(t)\\
        =&\sum_{u\in A(t)}\nabla_u F(h(t)\cdot\characteristic_{A(t)})\cdot h'(t)+\Big(\nabla_{v(t)} F(h(t)\cdot \characteristic_{A(t)})-\nabla_{u(t)}
F(h(t)\cdot\characteristic_{A(t)})\Big)\cdot h(t)
    \end{aligned}
    \end{equation}

where the gain of the value of $F$ comes from two parts: the first term comes from the increment of $h(t)$, and the second term comes from the random swap performed by the algorithm.



Conditioned on $R(t)\cap OPT\neq\emptyset$, since every element from $OPT$ appears uniformly at random in $R(t)$, $\pr{[v\in R(t)\mid R(t)\cap OPT\neq\emptyset]}\ge 1/r$ for every $v\in OPT$.
By Lemma \ref{le:perfect_matching_two_bases}, there exists a bijection $g:OPT\rightarrow A(t)$ such that $A(t)+v-g(v)\in \mathcal{I}$ for every $v\in OPT$. Because we choose the most beneficial swap (if any) in the algorithm, by averaging, the expected gain from the random swap satisfies
\[
\begin{aligned}
&\ex{\Big[\nabla_{v(t)} F(h(t)\cdot \characteristic_{A(t)})-\nabla_{u(t)}
F(h(t)\cdot\characteristic_{A(t)})\ \Big|\ R(t)\cap OPT\neq\emptyset \Big]}\\
\ge& \frac{1}{r}\sum_{v\in OPT}\Big(\nabla_{v} F(h(t)\cdot \characteristic_{A(t)})-\nabla_{g(v)}
F(h(t)\cdot\characteristic_{A(t)})\Big).
\end{aligned}
\]
Since every element appears independently uniformly at random with probability at least $1/\ell$, the probability that $R(t)$ contains at least one element from $OPT$ is at least $1-(1-1/\ell)^r\approx r/\ell$ when $\ell\rightarrow\infty$. Therefore,
\[
\begin{aligned}
\ex{\Big[\nabla_{v(t)} F(h(t)\cdot \characteristic_{A(t)})-\nabla_{u(t)}
F(h(t)\cdot\characteristic_{A(t)})\Big]}
\gtrsim& \frac{r}{\ell}\cdot \frac{1}{r}\sum_{v\in OPT}\Big(\nabla_{v} F(h(t)\cdot \characteristic_{A(t)})-\nabla_{g(v)}
F(h(t)\cdot\characteristic_{A(t)})\Big)\\
=& \frac{1}{\ell}\sum_{v\in OPT}\Big(\nabla_{v} F(h(t)\cdot \characteristic_{A(t)})-\nabla_{g(v)}
F(h(t)\cdot\characteristic_{A(t)})\Big).
\end{aligned}
\]

Plugging this into \eqref{eq:chain_rule}, one obtains
\begin{equation}\label{eq:iid_main}
\begin{aligned}
    \ex{\Big[\frac{d\, F(h(t)\cdot \characteristic_{A(t)})}{d\, t}\Big]}&
    \gtrsim \sum_{u\in A(t)}\nabla_u F(h(t)\cdot\characteristic_{A(t)})\cdot h'(t)+ \frac{h(t)}{\ell}\sum_{v\in OPT}\Big(\nabla_{v} F(h(t)\cdot \characteristic_{A(t)})-\nabla_{g(v)}
    F(h(t)\cdot\characteristic_{A(t)})\Big)\\
    \ge& \sum_{u\in A(t)}\nabla_u F(h(t)\cdot\characteristic_{A(t)})\cdot h'(t)+h'(t)\sum_{v\in OPT}\nabla_{v} F(h(t)\cdot \characteristic_{A(t)})-h'(t)\sum_{u\in A(t)}\nabla_u F(h(t)\cdot\characteristic_{A(t)})\\
    =& h'(t)\sum_{v\in OPT}\nabla_{v} F(h(t)\cdot \characteristic_{A(t)})\\
    \geq &h'(t)\cdot \Big(F(h(t)\cdot \characteristic_{A(t)} \vee \characteristic_{OPT})-F(h(t)\cdot \characteristic_{A(t)})\Big)\\
    \geq &h'(t)\cdot \Big(F(OPT)-F(h(t)\cdot \characteristic_{A(t)})\Big),
\end{aligned}
\end{equation}
where the second equality uses the fact that $h'(t)=\frac{h(t)}{\ell}$ so that the gain from the increment of $h(t)$ cancels out the loss of margins $\sum_{u\in A(t)}\nabla_u F$. This justifies the choice of $h$. The second inequality follows from the concavity of $F$ in the direction of $(h(t)\cdot\characteristic_{A(t)}\vee \characteristic_{OPT})-h(t)\cdot\characteristic_{A(t)}=0\vee (\characteristic_{OPT}-h(t)\cdot\characteristic_{A(t)})\ge 0$, where the notation $\vee$ means taking entry-wise maximum between two vectors. The third inequality is due to the monotonicity of $F$.

\nb{********}

Can we simply write that the solution to the differential equation: 

\begin{align*}
 \ex{\Big[\frac{d\, F(h(t)\cdot \characteristic_{A(t)})}{d\, t}\Big]} & \geq h'(t)\cdot \Big(F(OPT)-F(h(t)\cdot \characteristic_{A(t)})\Big) \\
 F(h(0) \cdot \characteristic_{A(0)}) & = F(h\cdot A)
\end{align*}

\[ F(h(t)\cdot\characteristic_{A(t)}) = (1-e^{-h(t)})\cdot f(OPT) + e^{-h(t)}\cdot F(h(0) \cdot \characteristic_{A(0)}) \]

Something is weird ...I'm confused.

\nb{******}



It follows that
\begin{equation}\label{eq:iid_DE}
    \begin{aligned}
    \ex{\Big[\frac{d\, \big(F(h(t)\cdot \characteristic_{A(t)})\cdot e^{h(t)}\big)}{d\, t}\Big]}
    =&\ex{\Big[\frac{d\, F(h(t)\cdot \characteristic_{A(t)})}{d\, t}\Big]}\cdot e^{h(t)}+ F(h(t)\cdot \characteristic_{A(t)})\cdot \frac{d\, e^{h(t)}}{d\, t}\\
    =&\ex{\Big[\frac{d\, F(h(t)\cdot \characteristic_{A(t)})}{d\, t}\Big]}\cdot e^{h(t)}+ F(h(t)\cdot \characteristic_{A(t)})\cdot h'(t)\cdot e^{h(t)}\\
    \gtrsim & h'(t)e^{h(t)} \cdot F(OPT),
\end{aligned}
\end{equation}
where the inequality follows from rearranging \eqref{eq:iid_main}. 

The final step follows from integrating from both sides in the following.
\[
\begin{aligned}
    \ex{\Big[F(e\cdot h\cdot \characteristic_{A(\ell)})\Big]}\cdot e^{e\cdot h}-F(h\cdot \characteristic_{A(0)})\cdot e^{h}
    =&\int_{t=0}^\ell \ex{\Big[d\, \big(F(h(t)\cdot \characteristic_{A(t)})\cdot e^{h(t)}\big)\Big]}\\
    \gtrsim& \int_{t=0}^\ell h'(t)e^{h(t)} \cdot F(OPT) \ d\, t\\
    =&F(OPT)\cdot \int_{t=0}^\ell d\, e^{h(t)}\\
    =&(e^{e\cdot h}-e^h)\cdot F(OPT).
\end{aligned}
\]
Dividing $e^{e\cdot h}$ from both sides, we obtain that
\[
\ex{[F(e\cdot h\cdot \characteristic_{A(\ell)})]}-F(h\cdot \characteristic_{A(0)})\cdot e^{-h(e-1)}\gtrsim (1-e^{-h(e-1)})\cdot F(OPT).
\]
\end{proof}

\subsection{Semi-streaming algorithm}
In the setting where elements arrive in a random stream, the property that every element $v\in OPT$ arrives at each time step with some positive probability $\frac{1}{\ell}$ is no longer true. Indeed, if an element $v\in OPT$ appears in a previous time step, it will never appear again. In order to address negative correlation cross time steps, we use an idea from \cite{agrawal2018submodular,feldman2026streaming,liu2021cardinality} that stores previously selected elements and makes them reappear in the stream. By partitioning $\cal{N}$ into $\ell$ random-sized windows we mean that each element in $\cal{N}$ appears independently and uniformly at random in each window (see Algorithm 4 in \cite{feldman2026streaming}). The algorithm that achieves Proposition \ref{prop:main} is the following.

\begin{algorithm}
\caption{\textsc{Single-Pass with Boosting}} \label{alg:multi-pass-one-pass}
\KwIn{A basis $A$ and a value $h\in [0,1/e]$}
Partition the stream into $\ell:=r/\delta$ randomly-sized windows $w_1,...,w_\ell$. \\
Let $H=\emptyset$.\\
\For{$i = 1$ \KwTo $\ell$}
{
    Let $R_i$ be a random set obtained from sampling each $u\in H$ independently with probability $\delta/k$.\\
    Let $h_i=h\cdot e^{i/\ell}$.\\
    Pick $u\in A$ and $v\in R_i\cup w_i$ such that $A-u+v\in\cal{I}$ and $F(h_{i}\cdot \characteristic_{A-u+v})$ is maximized.\\
    \If{$F(h_{i}\cdot \characteristic_{A-u+v})>F(h_{i}\cdot \characteristic_{A})$}
    {
    Let $A\gets A-u+v$.\\
    Update $H\gets H+u$
    }
}
\Return $A$.
\end{algorithm}

Denote as $H_i$ the set $H$ after the $i$-th iteration of the algorithm. Denote as $A_i$ the set $A$ after the $i$-th iteration of the algorithm.  Denote as $\mathcal{H}_i=\{(v,j):v\in H_i\cap w_j\}$, which is the ``history" that encodes when an element $v$ is added to $H_i$. Note that a fixed history $\mathcal{H}_{i}$ uniquely defines $A_i$, since the element $u$ removed from the solution when $v$ is added is deterministic (assuming we fix a rule of tie-breaking). The following lemma is from \cite{liu2021cardinality}. 
\begin{lemma}\label{lemma:opt_prob}
    Fix a history $\mathcal{H}_{i-1}$ for some $i \in [\ell]$. For any element $u \in \mathcal{N} \setminus H_{i-1}$, and any $i \le j \le \ell$, we have $\Pr[u \in w_j] \geq \frac{1}{\ell}$.
\end{lemma}
Note that the probability should be conditioned on the history $\mathcal{H}_{i-1}$, which we omit for brevity. We prove the following lemma.
\begin{lemma}\label{lemma:gain_F}
Fix a history $\mathcal{H}_{i-1}$ for some $i\in [\ell]$. For sufficiently small $\delta>0$, 
    \[\ex{[F(h_{i}\cdot\characteristic_{A_{i}})]}-F(h_{i-1}\cdot\characteristic_{A_{i-1}})\ge \frac{h_{i-1}}{\ell}(1-\frac{\delta}{2}) \Big(F(OPT)-F(h_{i}\cdot\characteristic_{A_{i-1}})-\sum_{u\in A_{i-1}}\nabla_{u} F(h_{i-1}\cdot\characteristic_{A_{i-1}})\Big).\]
\end{lemma}
\begin{proof}
It follows from Lemma \ref{lemma:opt_prob} and the definition of $R_i$ that for each iteration $i$, every element $u\in \cal{N}$ appears in $R_i\cup w_i$ with probability at least $\frac{1}{\ell}$. Therefore, the probability that $R_i\cup w_i$ contains at least one element from $OPT$ is at least $1-(1-1/\ell)^r=1-(1-\delta/r)^r\ge 1-1/e^\delta\ge \delta-\delta^2/2$. \siyue{This uses independence, so the proof is not rigorous... Need to use the active set approach in Moran's paper.}
Since every element from $OPT$ appears uniformly at random in $R_i\cup w_i$, $\pr{[v\in R_i\cup w_i\mid (R_i\cup w_i)\cap OPT\neq\emptyset]}\ge \frac{1}{r}$ for every $v\in OPT$.
By Lemma \ref{le:perfect_matching_two_bases}, there exists a bijection $g:OPT\rightarrow A_{i-1}$ such that $A_{i-1}+v-g(v)\in \mathcal{I}$ for every $v\in OPT$. Conditioned on $(R_i\cup w_i)\cap OPT\neq\emptyset$, 
\[
    \ex{[F(h_{i}\cdot\characteristic_{A_{i}})\mid (R_i\cup w_i)\cap OPT\neq\emptyset]}-F(h_{i}\cdot\characteristic_{A_{i-1}})
    \ge \frac{1}{r}\sum_{v\in OPT}\Big(F(h_{i}\cdot\characteristic_{A_{i-1}+v-g(v)})-F(h_{i}\cdot\characteristic_{A_{i-1}})\Big).
\]
This is because we choose the most beneficial swap (if any) in the algorithm. Then,
% \[
% \begin{aligned}
% \ex{[F(h_{i}\cdot\characteristic_{A_{i}})]}-F(h_{i}\cdot\characteristic_{A_{i-1}})
%     \ge& \delta(1-2\delta)\cdot\frac{1}{r}\sum_{v\in OPT}\Big(F(h_{i}\cdot\characteristic_{A_{i-1}+v-g(v)})-F(h_{i}\cdot\characteristic_{A_{i-1}})\Big)\\ =& \frac{1}{\ell}(1-2\delta)\sum_{v\in OPT}\Big(F(h_{i}\cdot\characteristic_{A_{i-1}+v-g(v)})-F(h_{i}\cdot\characteristic_{A_{i-1}})\Big).
% \end{aligned}
% \]
\[
\begin{aligned}
\ex{[F(h_{i}\cdot\characteristic_{A_{i}})]}-F(h_{i}\cdot\characteristic_{A_{i-1}})
    \ge& \delta(1-\frac{\delta}{2})\cdot\frac{1}{r}\sum_{v\in OPT}\Big(F(h_{i}\cdot\characteristic_{A_{i-1}+v-g(v)})-F(h_{i}\cdot\characteristic_{A_{i-1}})\Big)\\ =& \frac{1}{\ell}(1-\frac{\delta}{2})\sum_{v\in OPT}\Big(F(h_{i}\cdot\characteristic_{A_{i-1}+v-g(v)})-F(h_{i}\cdot\characteristic_{A_{i-1}})\Big).
\end{aligned}
\]
It follows that
\begin{equation}\label{eq:gain_swap}
\begin{aligned}
\ex{[F(h_{i}\cdot\characteristic_{A_{i}})]}-F(h_{i}\cdot\characteristic_{A_{i-1}})
\ge &\frac{h_{i-1}}{h_{i}}\big(\ex{[F(h_{i}\cdot\characteristic_{A_{i}})]}-F(h_{i}\cdot\characteristic_{A_{i-1}})\big)\\
\ge & \frac{1}{\ell}(1-\frac{\delta}{2})\frac{h_{i-1}}{h_{i}}\sum_{v\in OPT}\Big(F(h_{i}\cdot\characteristic_{A_{i-1}+v-g(v)})-F(h_{i}\cdot\characteristic_{A_{i-1}})\Big)\\
\ge &\frac{h_{i-1}}{\ell}(1-\frac{\delta}{2})\sum_{v\in OPT}\Big(\nabla_v F(h_{i}\cdot\characteristic_{A_{i-1}})-\nabla_{g(v)} F(h_{i}\cdot\characteristic_{A_{i-1}})\Big)\\  
=&\frac{h_{i-1}}{\ell}(1-\frac{\delta}{2})\Big(\sum_{v\in OPT}\nabla_v F(h_{i}\cdot\characteristic_{A_{i-1}})-\sum_{u\in A_{i-1}}\nabla_{u} F(h_{i}\cdot\characteristic_{A_{i-1}})\Big)\\
\ge &\frac{h_{i-1}}{\ell}(1-\frac{\delta}{2})\Big(F(h_{i}\cdot\characteristic_{A_{i-1}}\vee \characteristic_{OPT})-F(h_{i}\cdot\characteristic_{A_{i-1}})-\sum_{u\in A_{i-1}}\nabla_{u} F(h_{i}\cdot\characteristic_{A_{i-1}})\Big)\\
\ge &\frac{h_{i-1}}{\ell}(1-\frac{\delta}{2})\Big(F(OPT)-F(h_{i}\cdot\characteristic_{A_{i-1}})-\sum_{u\in A_{i-1}}\nabla_{u} F(h_{i}\cdot\characteristic_{A_{i-1}})\Big)\\
\ge &\frac{h_{i-1}}{\ell}(1-\frac{\delta}{2})\Big(F(OPT)-F(h_{i}\cdot\characteristic_{A_{i-1}})-\sum_{u\in A_{i-1}}\nabla_{u} F(h_{i-1}\cdot\characteristic_{A_{i-1}})\Big),
\end{aligned}
\end{equation}
where the first inequality follows from the fact that $h_{i-1}\le h_{i}$ and $\ex{[F(h_{i}\cdot\characteristic_{A_{i}})]}-F(h_{i}\cdot\characteristic_{A_{i-1}})\ge 0$. The second inequality is due to the discussion above. The third inequality follows from the convexity of $F$ in the direction of $\characteristic_v-\characteristic_u$ for every $u,v\in \cal{N}$. The fourth inequality follows from the concavity of $F$ in the direction of $(h_{i}\cdot\characteristic_{A_{i-1}}\vee \characteristic_{OPT})-h_{i}\cdot\characteristic_{A_{i-1}}=0\vee (\characteristic_{OPT}-h_{i}\cdot\characteristic_{A_{i-1}})\ge 0$, where the notation $\vee$ means taking entry-wise maximum between two vectors. The fifth inequality is due to the monotonicity of $F$. The last inequality follows from the fact that $\nabla_uF$ is non-increasing due to the submodularity of $f$.


Moreover, it follows from the concavity of $F$ in the direction $h_{i}\cdot \characteristic_{A_{i-1}}-h_{i-1}\cdot \characteristic_{A_{i-1}}=(h_{i}-h_{i-1})\characteristic_{A_{i-1}}\ge 0$ that
\begin{equation}\label{eq:gain_h}
    \begin{aligned}
    F(h_{i}\cdot \characteristic_{A_{i-1}})-F(h_{i-1}\cdot \characteristic_{A_{i-1}})
    \ge& (h_{i}-h_{i-1})\sum_{u\in A_{i-1}} \nabla_u F(h_{i}\cdot \characteristic_{A_{i-1}})\\
    =& h_{i-1}\big(e^{\frac{1}{\ell}}-1\big)\sum_{u\in A_{i-1}} \nabla_u F(h_{i}\cdot \characteristic_{A_{i-1}})\\
    \ge& \frac{h_{i-1}}{\ell}\sum_{u\in A_{i-1}} \nabla_u F(h_{i}\cdot \characteristic_{A_{i-1}}).
\end{aligned}
\end{equation}

Summing up \eqref{eq:gain_swap} and \eqref{eq:gain_h}, we obtain that
\[
\ex{\big[F(h_{i}\cdot \characteristic_{A_{i}})\big]}-F(h_{i-1}\cdot \characteristic_{A_{i-1}})\ge \frac{h_{i-1}}{\ell}(1-\frac{\delta}{2}) \big(F(OPT)-F(h_{i}\cdot\characteristic_{A_{i-1}})\big). 
\]
\end{proof}



% The next lemma is routine.
% \begin{lemma}\label{lemma:gain_h}
%     For every $i\in [\ell]$ and sufficiently small $\delta>0$, 
%     \[
%     F(h_{i}\cdot\characteristic_{A_{i-1}})-F(h_{i-1}\cdot\characteristic_{A_{i-1}})\ge \frac{h_{i-1}}{\ell}(1-2\delta)\sum_{u\in A_{i-1}} \nabla_u F(h_{i-1}\cdot \characteristic_{A_{i-1}}).
%     \]
% \end{lemma}
% \begin{proof}
%     Let $R$ be a random subset of $A_{i-1}$ where for every $j\in A_{i-1}$, $j$ is sampled independently with probability $h_{i-1}$. Let $D$ be a random subset of $A_{i-1}$ where for every $j\in A_{i-1}$, $j$ is sampled independently with probability $h_{i}-h_{i-1}$. Then, we claim that
%     \[
%     F(h_{i}\cdot\characteristic_{A_{i-1}})\geq \ex{[f(R\cup D)]}.
%     \]
%     Indeed, define $R'$ as a random subset of $A_{i-1}$ where for every $j\in A_{i-1}$, $j$ is sampled independently with probability $h_{i}$. Then, $\pr{[j\in R\cup D]}=1-(1-h_{i-1})(1-(h_{i}-h_{i-1}))\le h_{i}=\pr{[j\in R']}$. Thus, we may assume that $R\cup D\subseteq R'$ by coupling the two distributions. Therefore, $F(h_{i}\cdot\characteristic_{A_{i-1}})=\ex{[f(R')]}\ge \ex{[f(R\cup D)]}$, as claimed. Therefore,
% \[
% \begin{aligned}
%     F(h_{i}\cdot\characteristic_{A_{i-1}})-F(h_{i-1}\cdot\characteristic_{A_{i-1}})
%     \geq &\ex{[f(R\cup D)-f(R)]}\\
%     \geq &\sum_{u\in A_{i-1}}\pr{[D=\{u\}]}\cdot \ex{[f(u\mid R)]}\\
%     =&\big(h_{i}-h_{i-1}\big)\big(1-(h_{i}-h_{i-1})\big)^{r-1} \sum_{u\in A_{i-1}}\nabla_u F(h_{i-1}\cdot \characteristic_{A_{i-1}})\\
%     \geq &\big(h_{i}-h_{i-1}\big)\big(1-(r-1)(h_{i}-h_{i-1})\big) \sum_{u\in A_{i-1}} \nabla_u F(h_{i-1}\cdot \characteristic_{A_{i-1}})\\
%     \geq &h_{i-1}\big(e^{\frac{1}{\ell}}-1\big)\big(1-r(e^{\frac{1}{\ell}}-1)\big)\sum_{u\in A_{i-1}} \nabla_u F(h_{i-1}\cdot \characteristic_{A_{i-1}})\\
%     \geq &\frac{h_{i-1}}{\ell}\big(1-\frac{2r}{\ell}\big)\sum_{u\in A_{i-1}} \nabla_u F(h_{i-1}\cdot \characteristic_{A_{i-1}})\\
%     = &\frac{h_{i-1}}{\ell}(1-2\delta)\sum_{u\in A_{i-1}} \nabla_u F(h_{i-1}\cdot \characteristic_{A_{i-1}}),
% \end{aligned}
% \]
% where the second inequality holds because we only calculated the contribution of $f(D\mid R)$ when $D$ is a singleton. In the third inequality we used that $h_{i}-h_{i-1}=h_{i-1}(e^{\frac{1}{\ell}}-1)\le e^{\frac{1}{\ell}}-1$. In the fourth inequality we used the fact that $e^{\frac{1}{\ell}}-1\le \frac{2}{\ell}$, which holds for sufficiently small $\delta=r/\ell$.
% \end{proof}

\begin{lemma}\label{lemma:recursion_hA}
Fix a history $\mathcal{H}_{i-1}$ for some $i\in [\ell]$. For sufficiently small $\delta>0$,
    \[\ex{\big[F(h_{i}\cdot \characteristic_{A_{i}})\big]}\cdot e^{h_{i}}-F(h_{i-1}\cdot \characteristic_{A_{i-1}})\cdot e^{h_{i-1}}\ge (e^{h_{i}}-e^{h_{i-1}})(1-4\delta)\cdot F(OPT)\]
\end{lemma}
\begin{proof}
% Combining Lemmas \ref{lemma:gain_swap} and \ref{lemma:gain_h}, we obtain that
% \begin{equation}\label{eq:gain_F}
%    \ex{\big[F(h_{i}\cdot \characteristic_{A_{i}})\big]}-F(h_{i-1}\cdot \characteristic_{A_{i-1}})\ge \frac{h_{i-1}}{\ell}(1-2\delta) \big(F(OPT)-F(h_{i}\cdot\characteristic_{A_{i-1}})\big). 
% \end{equation}
% Thus, it follows that

\begin{equation}\label{eq:gain_hA}
\begin{aligned}
    &\ex{\big[F(h_{i}\cdot \characteristic_{A_{i}})\big]}\cdot e^{h_{i}}-F(h_{i-1}\cdot \characteristic_{A_{i-1}})\cdot e^{h_{i-1}}\\
    = &\ex{\big[F(h_{i}\cdot \characteristic_{A_{i}})\big]}\cdot (e^{h_{i}}-e^{h_{i-1}})+\big(\ex{\big[F(h_{i}\cdot \characteristic_{A_{i}})\big]}-F(h_{i-1}\cdot \characteristic_{A_{i-1}})\big)\cdot e^{h_{i-1}}\\
    \ge &\ex{\big[F(h_{i}\cdot \characteristic_{A_{i}})\big]}\cdot (e^{h_{i}}-e^{h_{i-1}})+\frac{h_{i-1}}{\ell}(1-2\delta) \big(F(OPT)-F(h_{i}\cdot\characteristic_{A_{i-1}})\big)\cdot e^{h_{i-1}}\\
    \ge &F(h_{i}\cdot \characteristic_{A_{i-1}})\cdot (e^{h_{i}}-e^{h_{i-1}})+\frac{h_{i-1}}{\ell}(1-2\delta) \big(F(OPT)-F(h_{i}\cdot\characteristic_{A_{i-1}})\big)\cdot e^{h_{i-1}}\\
    = &F(h_{i}\cdot \characteristic_{A_{i-1}})\cdot e^{h_{i-1}}\cdot (e^{h_{i-1}(e^{\frac{1}{\ell}}-1)}-1)+\frac{h_{i-1}}{\ell}(1-2\delta) \big(F(OPT)-F(h_{i}\cdot\characteristic_{A_{i-1}})\big)\cdot e^{h_{i-1}}\\
    \ge &F(h_{i}\cdot \characteristic_{A_{i-1}})\cdot e^{h_{i-1}}\cdot h_{i-1}(e^{\frac{1}{\ell}}-1)+\frac{h_{i-1}}{\ell}(1-2\delta) \big(F(OPT)-F(h_{i}\cdot\characteristic_{A_{i-1}})\big)\cdot e^{h_{i-1}}\\
    \ge &F(h_{i}\cdot \characteristic_{A_{i-1}})\cdot e^{h_{i-1}}\cdot \frac{h_{i-1}}{\ell}+\frac{h_{i-1}}{\ell}(1-2\delta) \big(F(OPT)-F(h_{i}\cdot\characteristic_{A_{i-1}})\big)\cdot e^{h_{i-1}}\\
    \ge& \frac{h_{i-1}}{\ell} e^{h_{i-1}}(1-2\delta)\cdot F(OPT).
\end{aligned}
\end{equation}
where the first inequality is due to \Cref{lemma:gain_F}, and the second inequality follows from the fact that the algorithm only carries beneficial swaps. Moreover, using the fact that $e^x\leq \frac{1}{1-x}$ for every $x<1$, we obtain that
\[
\begin{aligned}
    e^{h_{i}}-e^{h_{i-1}}=&e^{h_{i-1}}(e^{h_{i-1}(e^{\frac{1}{\ell}}-1)}-1)\le e^{h_{i-1}}\cdot \Big(\frac{1}{1-h_{i-1}(e^{\frac{1}{\ell}}-1)}-1\Big)\\
    \le& e^{h_{i-1}}\cdot\Big(\frac{1}{1-h_{i-1}\big(\frac{1}{1-\frac{1}{\ell}}-1\big)}-1\Big)=e^{h_{i-1}}\cdot \frac{h_{i-1}}{\ell-1-h_{i-1}}\le e^{h_{i-1}}\cdot \frac{h_{i-1}}{\ell-2}.
\end{aligned}
\]
Therefore, 
\[
\begin{aligned}
    \frac{h_{i-1}}{\ell} e^{h_{i-1}}(1-2\delta)\ge (e^{h_{i}}-e^{h_{i-1}})(1-\frac{2}{\ell})(1-2\delta)\ge (e^{h_{i}}-e^{h_{i-1}})(1-2\delta)^2\ge (e^{h_{i}}-e^{h_{i-1}})(1-4\delta).
\end{aligned}
\]
Combining this with \eqref{eq:gain_hA}, we obtain the desired inequality in this Lemma.
\end{proof}

Finally, we complete the proof of Proposition \ref{prop:main}.
\begin{proof}[Proof of Proposition \ref{prop:main}]
Using Lemma \ref{lemma:recursion_hA} and taking expectations over all histories $\mathcal{H}_{i-1}$ for every $i\in[\ell]$, we obtain that
    \[
    \begin{aligned}
    \ex{\big[F(h_{\ell}\cdot \characteristic_{A_{\ell}})\big]}\cdot e^{h_{\ell}}-F(h_{0}\cdot \characteristic_{A_{0}})\cdot e^{h_{0}}=&\sum_{i=1}^{\ell}\Big(\ex{\big[F(h_{i}\cdot \characteristic_{A_{i}})\big]}\cdot e^{h_{i}}-\ex{\big[F(h_{i-1}\cdot \characteristic_{A_{i-1}})\big]}\cdot e^{h_{i-1}}\Big)\\
    \ge& \sum_{i=1}^{\ell}(e^{h_{i}}-e^{h_{i-1}})(1-4\delta)\cdot F(OPT)\\
    =&(e^{h_{\ell}}-e^{h_{0}})(1-4\delta)\cdot F(OPT).
    \end{aligned}
    \]
    Since $h_\ell=e\cdot h_0=e\cdot h$, we have
    \[
    \ex{\big[F(e\cdot h\cdot \characteristic_{A_{\ell}})\big]}\cdot e^{e\cdot h}-F(h\cdot \characteristic_{A_{0}})\cdot e^{h}\ge (e^{e\cdot h}-e^{h})(1-4\delta)\cdot F(OPT).
    \]
    Dividing $e^{h_\ell}=e^{h_0\cdot e}=e^{h\cdot e}$ from both sides and rearranging, we obtain tat
    \[
    \ex{\big[F(e\cdot h\cdot \characteristic_{A_{\ell}})\big]}\ge (1-e^{-h(e-1)})(1-4\delta)\cdot F(OPT)+e^{-h(e-1)} \cdot F(h\cdot \characteristic_{A_{0}}),
    \]
    which is the desired inequality for the second part of Proposition \ref{prop:main}. Observe that we only store the set $H$, which consists of at most one element per window. Therefore, the space requirement is at most $\ell=O(r/\delta)$.

    The first part of Proposition \ref{prop:main} follows from observing the following and plugging in $h=1/e$.
    \[
    F(h\cdot \characteristic_A)\ge h\cdot (1-h)\cdot f(\emptyset)+h\cdot f(A)\ge h\cdot f(A),
    \]
    where the first inequality follows from the concavity of $F$ in the direction of $\characteristic_A$, and the second inequality follows from the nonnegativity of $f$.
\end{proof}




==> niv-sketch-iid.tex <==
\subsection{OLD *****}

We have the following lemma from our previous paper \nb{we only need several}

\begin{lemma} \label{lem:DR_properties}
Let $F\colon [0, 1]^\cN \to \nnR$ be a non-negative differentiable DR-submodular function. Then,
\begin{enumerate}
	\item $F(\lambda \cdot \vx+(1-\lambda) \cdot \vy) \geq \lambda \cdot F(\vx) +(1-\lambda) \cdot F(\vy)$ for every two vectors $\vx,\vy \in [0, 1]^\cN$ such that $\vx \leq \vy$ and value $\lambda\in[0,1]$. \label{prop:dr_bound1}
	\item $F(\vx+\lambda \cdot \vy) -F(\vx) \geq \lambda \cdot \left(F(\vx+\vy) -F(\vx)\right)$ for every two vectors $\vx \in [0, 1]^\cN$ and $\vy \geq \vzero$ such that $\vx+\vy \leq \vone$ and $\lambda\in[0,1]$. \label{prop:dr_bound11}
	\item $\inner{\nabla F(\vx)}{\vy} \geq F(\vx+\vy) - F(\vx)$ for every $\vx\in [0, 1]^\cN$ and $\vy\geq \vzero$ such that $\vx+\vy \leq \vone$. \label{prop:dr_bound2_up}
	\item $\inner{\nabla F(\vx)}{\vy} \leq F(\vx) - F(\vx-\vy)$ for every $\vx\in [0, 1]^\cN$ and $\vy\geq \vzero$ such that $\vx-\vy \geq \vzero$. \label{prop:dr_bound2_down}
	\item $F(\vx \vee \vy) + F(\vx \wedge \vy) \geq F(\vx \psum \vy) + F(\vx \hprod \vy)$ for every two vectors $\vx, \vy \in [0, 1]^\cN$. \label{prop:old_new_notation}
\end{enumerate}
\end{lemma}



\begin{algorithm}
\caption{\textsc{Matroid offline algorithm}} \label{alg:iid2}
\KwIn{Matroid $(\cN, \cI)$ of rank $r$, non-negative monotone submodular function $f$, $A_0\in \cI$, parameters $h \in (0, 1)$. 
}
\smallskip\hrule\smallskip
Let $\ell \in [1, \log(\nicefrac{1}{h})/\log(1+\nicefrac{1}{(r-1)})]$ 
and $w\in [1,n]$.\\

\For{$i = 1$ \KwTo $\ell$}
{ 
Let $h_i=h \cdot (1+\nicefrac{1}{(r-1)})^{i}$.\\
Sample uniformly a set of random elements $R$, where $|R|=w$ (or $\bE[|R|]=w$).\\
Let $u= \arg \max_{u\in A_{i-1}, v\in R, A_{i-1}-u+v\in \cI} F(h_i \cdot \characteristic_{A_{i-1}-u+v})$.\\
\lIf{$F(h_i \cdot \characteristic_{A_{i-1}-u+v})>F(h_i \cdot \characteristic_{A_{i-1}})$}
    {
     $A_i\gets A_{i-1}-u+v$.
    } 
}
\Return $A_{\ell}$.
\end{algorithm}

\begin{observation}
By the choice of $\ell \leq \log(\nicefrac{1}{h})/\log(1+\nicefrac{1}{(r-1)})$, we have $h_{\ell} = h \cdot (1+\nicefrac{1}{(r-1)})^{\ell} \leq 1$    
\end{observation}

\begin{observation}
By the choice of $w$, the probability that we do not have any element of OPT in the sample $R$ is $\frac{{n-r\choose w}}{{n\choose w}}\leq (1-\frac{r}{n})^{w}$. Given that we have an element of OPT, it is a random element.    
\end{observation}

We next prove our main lemma. \nb{add expectation everywhere}
\begin{lemma}
Consider step $i$ of the algorithm and let $\Delta h_{i} = h_i - h_{i-1}$. Then, if the sample contains a random element of OPT, then we have
\begin{equation}
(1+\Delta h_i) \cdot F(h_i \cdot \characteristic_{A_i})  
  \geq \Delta h_{i} \cdot f(OPT) + F(h_{i-1} \cdot \characteristic_{A_{i-1}}) \label{eq-offline-step}
\end{equation}
\end{lemma}

\begin{proof}
Suppose the sample contains an element of OPT. We have
\[F(h_i \cdot \characteristic_{A_i}) - F(h_{i-1} \cdot \characteristic_{A_{i-1}}) = \big[F(h_i \cdot \characteristic_{A_i}) - F(h_i \cdot \characteristic_{A_{i-1}})\big] + \big[F(h_i \cdot \characteristic_{A_{i-1}}) - F(h_{i-1} \cdot \characteristic_{A_{i-1}})\big]\]
Hence, we partition the analysis into two steps. 
\paragraph{Analysis of the term $\big[F(h_i \cdot \characteristic_{A_{i-1}}) - F(h_{i-1} \cdot \characteristic_{A_{i-1}})\big]$:}
\begin{align*}
    F(h_i \cdot \characteristic_{A_{i-1}})-F(h_{i-1} \cdot \characteristic_{A_{i-1}}) & = F(h_i \cdot \characteristic_{A_{i-1}})-F(h_i\cdot \characteristic_{A_{i-1}} -\Delta h_i \cdot \characteristic_{A_{i-1}}) \geq \Delta h_i \cdot \inner{\nabla F(h_i \cdot \characteristic_{A_{i-1}})}{ \characteristic_{A_{i-1}}}
\end{align*}
We use: $\inner{\nabla F(\vx)}{\vy} \leq F(\vx) - F(\vx-\vy)$ for every $\vx\in [0, 1]^\cN$ and $\vy\geq \vzero$ such that $\vx-\vy \geq \vzero$.

\paragraph{Analysis of the term $\big[F(h_i \cdot \characteristic_{A_i}) - F(h_i \cdot \characteristic_{A_{i-1}})\big]$:}
By Corollary \ref{cor:perfect_matching_two_bases} there is a bijection  $g\colon O \rightarrow A_{i-1}$ such that for every $o \in O$, $(A_{i-1} - g(o)) + o \in \cI$ and $h(o) =o$ for every $o\in A_{i-1}\cap O$. 
\begin{align}
 \lefteqn{   F(h_i \cdot \characteristic_{A_{i}})-F(h_i \cdot \characteristic_{A_{i-1}})} \nonumber \\ & \geq \frac{1}{r}\cdot \sum_{o\in O}\left[F(h_i \cdot \characteristic_{A_{i-1}-g(o)+o})-  F(h_i \cdot \characteristic_{A_{i-1}})\right] \nonumber \\
    & \geq  \frac{h_i}{r}\cdot \sum_{o\in O}\left[F(h_i \cdot \characteristic_{A_{i-1}} \vee \characteristic_{o})- F(h_i \cdot \characteristic_{A_{i-1}})\right] - \frac{h_i}{r}\cdot \inner{\nabla F(h_i \cdot \characteristic_{A_{i-1}})}{ \characteristic_{A_{i-1}}} \label{ineq-11}\\
    & \geq \frac{h_i}{r}\cdot \left[f(OPT)- F(h_i \cdot \characteristic_{A_{i-1}})\right] - \frac{h_i}{r}\cdot \inner{\nabla F(h_i \cdot \characteristic_{A_{i-1}})}{ \characteristic_{A_{i-1}}} \nonumber\\
    & = \Delta h_i \cdot \left[f(OPT)- F(h_i \cdot \characteristic_{A_{i-1}})\right] - \Delta h_i \cdot \inner{\nabla F(h_i \cdot \characteristic_{A_{i-1}})}{ \characteristic_{A_{i-1}}} \label{ineq-12}
\end{align}
\nb{We can multiply by $q\in [0,1]$ the term \[F(h_i \cdot \characteristic_{A_{i}})-F(h_i \cdot \characteristic_{A_{i-1}}) \nonumber \geq q \cdot \frac{1}{r}\cdot \sum_{o\in O}\left[F(h_i \cdot \characteristic_{A_{i-1}-g(o)+o})-  F(h_i \cdot \characteristic_{A_{i-1}})\right]\] Then, we will need $-q \frac{h}{r}\geq \Delta h$. Then, we can make $\Delta h = q \frac{h}{r}$ ... smaller steps for $\eps \leq 1/r$. Should we take $q=\eps$?
}

The first inequality follows as the sample contains a random element of OPT and the algorithm chooses the best swap. 
Inequality \eqref{ineq-11} follows term by term since if $o\in O \setminus A_{i-1}$ then, by submodularity, the LHS is at most
\begin{align*}
& F(h_i \cdot \characteristic_{A_{i-1}+o})- F(h_i \cdot \characteristic_{A_{i-1}}) - \bigg(F(h_i \cdot \characteristic_{A_{i-1}})-F(h_i \cdot \characteristic_{A_{i-1}-u})\bigg)\\
& = h_i \cdot \big(F(h_i \cdot \characteristic_{A_{i-1}} \vee \characteristic_{o})- F(h_i \cdot \characteristic_{A_{i-1}})\big) - h_i \cdot 
\frac{\partial F(h_i \cdot \characteristic_{A_{i-1}}))}{\partial u}
,   
\end{align*}
If $o\in O \cap A_{i-1}$ ($g(o)=o=u$) then the LHS of Inequality \eqref{ineq-11} is zero for such an element, while the RHS is 
\[h_i \cdot \big(F(h_i \cdot \characteristic_{A_{i-1}} \vee \characteristic_{o})- F(h_i \cdot \characteristic_{A_{i-1}})\big) - h_i \cdot 
\frac{\partial F(h_i \cdot \characteristic_{A_{i-1}}))}{\partial u} = -h_i^2 \cdot \frac{\partial F(h_i \cdot \characteristic_{A_{i-1}}))}{\partial u} \leq 0\]
\nb{Right? we have slack here??}
Finally, Inequality \eqref{ineq-12} follows as $h_i= h_{i-1}\cdot (1+\nicefrac{1}{r-1}) = h_{i-1} \cdot \frac{r}{r-1}$ and so $\Delta h_i = h_{i-1}\cdot \frac{1}{r-1}= \frac{h_i}{r}$. 
The lemma follows by adding both terms. 
\end{proof}

Using complete probability and the fact that $F(h_i \cdot \characteristic_{A_i}) \geq F(h_{i-1} \cdot \characteristic_{A_{i-1}})$ we get the following:

\begin{corollary}
Consider step $i$ of the algorithm and let $\Delta h_{i} = h_i - h_{i-1}$. Let $p_G$ be the probability that the sample contains a random element of OPT then:
\begin{equation}
   (1+ p_G \cdot \Delta h_i) \cdot F(h_i \cdot \characteristic_{A_i})  
  \geq p_G\cdot \Delta h_{i} \cdot f(OPT) + F(h_{i-1} \cdot \characteristic_{A_{i-1}}) \label{eq-offline-step2} 
\end{equation}
\end{corollary}

\begin{proof}
    Sketch:
    \[p\bigg[(1+\Delta h_i) \cdot F(h_i \cdot \characteristic_{A_i})  
  - \Delta h_{i} \cdot f(OPT) - F(h_{i-1} \cdot \characteristic_{A_{i-1}})\bigg] + (1-p)\bigg[ F(h_i \cdot \characteristic_{A_i}) - F(h_{i-1} \cdot \characteristic_{A_{i-1}})\bigg] \geq 0\]
\end{proof}

By solving the recursion we have the following:
\begin{corollary}
If the sample contains a random element of OPT with probability $p_G$ then We have,
\begin{align*}
F(h_i \cdot \characteristic_{A_i}) & \geq  \bigg(1- \frac{1}{\prod_{j=1}^{i}(1+p_G\cdot \Delta h_i)} \bigg) \cdot f(OPT)+ \frac{1}{\prod_{j=1}^{i}(1+p_G\cdot \Delta h_i)} \cdot F(h \cdot \characteristic_{A_{0}}) \\
& \geq   \bigg(1- e^{-p_G \cdot \sum_{j=1}^{i}\Delta h_i+\frac{1}{2}\sum_{j=1}^{i}(p_G \cdot \Delta h_i)^2} \bigg) \cdot f(OPT)
\end{align*}
\end{corollary}

\nb{is the last inequality correct? helpful? we use $\ln(1+x)\geq x-x^2/2$ (for $x\geq 0$}

\begin{proof}
Rearranging Inequality \eqref{eq-offline-step2} we have:
\[F(OPT)- F(h_i \cdot \characteristic_{A_i}) \leq \frac{1}{1+p_G\cdot \Delta h_i}\cdot \left(f(OPT) - F(h_{i-1} \cdot \characteristic_{A_{i-1}})\right)\]

Therefore, by induction we get \[F(OPT)- F(h_i \cdot \characteristic_{A_i}) \leq \bigg(f(OPT) - F(h \cdot \characteristic_{A_{0}})\bigg)\cdot \frac{1}{\prod_{j=1}^{i}(1+p_G\cdot \Delta h_i)}\]  
\end{proof}

\nb{Is the following lemma correct? Is this the result in \cite{ganz2026poisson}? the less oracle calls is with our optimization for local search.}

Computations. Suppose we take $p_G=1$, $h_0=\eps$. We have $\Delta h_i = \frac{h_i}{r} = \frac{\eps}{r} \cdot (1+\nicefrac{1}{(r-1)})^{i} = \frac{\eps}{r} \cdot c^i$.
We use $h_{\ell}=\eps c^{\ell}=1$ (so $c^{\ell}=1/\eps$).
We have $\sum_{i=1}^{\ell}\Delta h_i \geq 1-\eps$. 
We have:
\begin{align*}
 \sum_{i=1}^{\ell}(\Delta h_i)^2 & = (\frac{\eps}{r})^2\sum_{i=1}^{\ell}c^{2i} \leq (\frac{\eps}{r})^2\cdot \frac{c^{2\ell}}{c^2-1} = \frac{1}{r^2} \cdot \frac{1}{c^2-1} = \frac{1}{r^2} \cdot \frac{1}{(1+\nicefrac{1}{(r-1)})^2-1} \approx \frac{2}{r}
\end{align*}

Suppose we have $\eps>\frac{1}{r}$, then this is at most $2\eps$. If $\eps<1/r$ the complexity is $poly(r)$?? \nb{what should we do?}
If $\eps<1/r$, we should use $\eps=1/2r$, but guess a single element of OPT and then get $1-1/e$??


\nb{***}


\begin{lemma}
Algorithm \ref{alg:iid2} with parameters $h=\eps$, $\ell = \log(\nicefrac{1}{\eps})/\log(1+\nicefrac{1}{(r-1)}) = O(r \cdot \log(\nicefrac{1}{\eps}))$, $w=\frac{n}{r}\cdot \log(\nicefrac{1}{\eps})$, we get an $\frac{e}{e-1}+\eps$-approximation. The algorithm performs  $O(n \log^2 (1/\eps)$ value oracle calls {\bf to $F$} and $O(r\log(1/\eps))$ swaps.
\end{lemma}
\begin{proof}
\nb{Need to write. Sketch}
If we plug $h_0= \eps$ $h_i= \eps \cdot e^{i/r}$ Then, $\Delta h_i \approx \frac{\eps}{r} \cdot e^{i/r}$. We sum until $h_i= \eps \cdot e^{i/r} = 1$, so $\Delta h_i=1/r$ and $e^{i/r}=1/\eps$.

\[\prod_{j=1}^{i}(1+\frac{\eps}{r} \cdot e^{j/r}) \approx \prod_{j=1}^{i}e^{\frac{\eps}{r} \cdot e^{j/r}}= e^{\frac{\eps}{r} \cdot \sum_{j=1}^{i}e^{j/r}}\approx e^{\frac{\eps}{r} \cdot ((1/\eps)/(1/r))}\approx e\]    
\end{proof}

==> unknown-r.tex <==
\section{Handling Unknown Rank} \label{app:discovering_r}

The proof of Proposition~\ref{prop:main2} in Section~\ref{sec:single-pass} was based on an algorithm that gets as parameter the rank $r$ of the $p$-system constraint. In this section, our goal is to modify the proof of Proposition~\ref{prop:main2} so that it works also when $r$ is not known upfront. Our starting point is the observation that the analysis of the algorithm from Section~\ref{sec:single-pass} makes surprisingly little use of the property that the value of the parameter $r$ is indeed the rank of the $p$-system constraint. In fact, the only place in which this property is used is in the proof of Observation~\ref{obs:O_double_prime}, which uses this property to argue that the size of the set $S_r$ is upper bounded by $r$ whenever the set $O''_r$ is non-empty. Given this situation, we can deduce that the approximation guarantee of the algorithm from Section~\ref{sec:single-pass} holds whenever the parameter $r$ it gets is a strictly larger than the size of $S_r$, regardless of the relationship between $r$ and the true rank of the $p$-system constraint. Accordingly, most of this section is devoted to finding a method that is able to produce such a value for $r$ (with good probability) after inspecting only a small fraction of the data stream. It is important to note, however, that this method must also not over estimate the rank by too much because the space complexity of the algorithm from Section~\ref{sec:single-pass} grows with $r$.

Recall that the algorithm from Section~\ref{sec:single-pass} constructs $S_r$ while inspecting the first $\delta n$ elements of the data stream. Therefore, if we denote by $\cN'_1$ the set of these $\delta n$ elements, then the size of $S_r$ is upper bounded by the rank of $\cN'_1$, and estimating the rank of $\cN'_1$ is quite simple. To do that, one only needs to construct a base $B_1$ of $\cN'_1$ by starting with the empty set, and then greedily adding to $B_1$ every element of $\cN'_1$ whose addition preserves $B_1$'s independence. Since $(\cN, \cI)$ is a $p$-system, the rank of $\cN_1$ is upper bounded by $p \cdot |B_1|$. Thus, $p \cdot |B_1| + 1$ is always a good value for the parameter $r$, as it is always a strict upper bound on the size of $S_r$, which is the property that we need $r$ to obey. In practice, however, we cannot set $r$ to $p \cdot |B_1| + 1$ because this value is available to us too late. More specifically, to construct $S_r$, we need the value of the parameter $r$ to be known upfront, but the construction of $B_1$ requires us to scan all the elements of $\cN'_1$, and therefore, the value of $p \cdot |B_1| + 1$ is only available to us after the elements of $\cN'_1$ have already been processed.

A first attempt to bypass the above issue is to split the first $\delta n$ elements into two consecutive blocks of $\delta n / 2$ elements, which we denote by $\cN'_1$ and $\cN''_1$. Then, we can build $B_1$ as a base of $\cN'_1$ and use $p \cdot |B_1| + 1$ as the value for $r$ when constructing $S_r$ out of the elements of $\cN''_1$. One can note that this strategy works when the rank of $\cN'_1$ is at least as large as the rank of $\cN''_1$, which happens with probability at least $1/2$ since both sets are drawn from the same distribution. Unfortunately, however, a probability of $1/2$ is not good enough for us. To augment this probability, we need to split the first $\delta n$ elements into $2q = 2 \lceil \log_2 \delta^{-1}\rceil$ consecutive blocks denoted by $\cN'_1, \cN''_1, \cN'_2, \cN''_2, \dotsc, \cN'_q, \cN''_q$. Then, for every $h \in [q]$, we construct a base $B_h$ of $\cN'_h$ when the elements of $\cN'_h$ are processed, define $r_h \triangleq p \cdot |B_h| + 1$, and then use this value as the parameter $r$ when constructing a set $S_{h, r}$ using elements of $\cN''_h$. Notice that with probability at least $1 - \delta$ this strategy works in the sense that the rank of $\cN'_h$ is at least as large as the rank of $\cN''_h$ for some $h \in [q]$, which allows us to produce a good output solution based on the set $S_{h, r}$. The down side of this approach is that it somewhat increases the space complexity of the algorithm for three reasons: first, we need to store in $H$ elements that might be valuable with respect to each one of the sets $S_{h, r}$; second, each block $\cN''_h$ contains significantly less than $\delta n$ elements, which increases the probability that a given element is deemed as possibly valuable with respect to any given set $S_{h, r}$; and finally, the value $r_h$ can overestimate the true rank of the $p$-system constraint by about a factor of $p$.

The algorithm that is obtained using the approach described above is formally stated as Algorithm~\ref{alg:filter_no_r}. In this algorithm, we assume that $\delta n / (2q) = \delta n / (2 \lceil \log_2 \delta^{-1}\rceil)$ is an integer. If this is not the case, then this can always be fixed in one of two ways. If $\delta n / (2q) < 6$, then $n = O(\delta^{-1} q) = O(\delta^{-1} \log \delta^{-1})$, which is small enough so that we can return the entire stream as the set $H$. Otherwise, if $\delta n  (2q) > 6$, then we can always replacing $\delta$ with a value in the range $[\delta/2, \delta]$ for which $\delta n / (2q)$ is integer. Unfortunately, we cannot assume also that $\delta n / (2qr_h)$ is an integer for every $h \in [q]$, which somewhat complicates the technical presentation of Algorithm~\ref{alg:filter_no_r}. Recall that $\tilde{N}$ denotes the set of elements of the stream that are not among the first $\delta n$ elements.

\begin{algorithm}
\caption{\textsc{Filtering Streaming} (with unknown rank)} \label{alg:filter_no_r}
\DontPrintSemicolon
\KwIn{Independence system $(\cN, \cI)$, non-negative submodular function $f$, parameter $\delta \in(0,1)$. 
}
\smallskip\hrule\smallskip
\nonl\textbf{Inspecting the first $\delta n$ elements of the stream:} \\
Let $q \gets \lceil \log_2 \delta^{-1} \rceil$.\\
\For{$h \gets 1$ \KwTo $q$}
{
	Let $B_h \gets \varnothing$.\\
	\For{each element $u \in \cN''_h$}
	{
		\lIf{$B_h + u \in \cI$}{Add $u$ to $B_h$.}
	}
	Let $r_h \gets p \cdot |B_h| + 1$.\\
	For every $j \in [r_h]$, define $\cN''_{h, j}$ as the $j$-th block when $\cN''_{h, j}$ is divided into blocks of $\lfloor \delta n / (2qr_h) \rfloor$ consecutive elements each.\\
	Let $S_{h, 0} \gets \varnothing$.\\
\For{$j = 1$ \KwTo $r$}
{
Let $s_{h, j} \gets \arg \max_{u\in \cN''_{h, j}, S_{h,j-1}+u\in \cI, f(u \mid S_{h,j-1})\geq 0}f(u \mid S_{h,j-1})$.\label{line:choose_no_r}\\
\lIf{there is an element $s_{h, j}$}{Let $S_{h, j} \gets S_{h, j-1} + s_{h,j}$,}
\lElse{Let $S_{h, j} \gets S_{h, j - 1}$ and treat $f(s_{h, j} \mid S_{h, j - 1})$ as $0$.}
}
}
\Return the set maximizing $f$ among $S_{1, r_1}, S_{2, r_2}, \dotsc, S_{q, r_h}$.\\
\smallskip\hrule\smallskip
\nonl\textbf{Inspecting the remaining $(1-\delta)n$ elements of the stream:}\\
\If{$\delta n / (2qr_h) < 1$ for some $h \in [q]$}
{
	Return as $H$ the set of all the remaining $(1-\delta)n$ elements of the stream and terminate.
}
\For{$h \gets 1$ \KwTo $q$}
{
Let $k_h \gets \lceil 2\delta^{-1} \ln (r_h/\delta)\rceil$, and set
\begin{align*}
 v_{h, i}& \gets\frac{\max_{j=1}^{r_h}f(s_{h, j} \mid S_{h, j-1})}{(1+\delta)^i} &&  \forall\; i \in \{0, 1, \ldots, k_h\} \enspace, \quad\text{and} \\ 
 w_{h, j} & \gets \min\{v_{h, i} \mid v_{h, i}\geq f(s_{h, j} \mid S_{h, j-1})\} && \forall\; j \in \{1, 2, \ldots, r_h\} \enspace.
\end{align*}
}
Let $H \gets \cup_{h = 1}^q \cup_{j=1}^{r_h}\{u\in \tilde{\cN}, S_{h, j-1}+u\in \cI, f(u \mid S_{h, j-1})> w_{h, j}\}$.\\
\lIf{$|H|\leq \sum_{h = 1}^q 4r_h\delta^{-2} \ln^2 (\nicefrac{r_h}{\delta})$}{\Return $H$, }\lElse{\Return $\varnothing$ and indicate failure.}
%\Return $(S_r, H)$.
\end{algorithm}
